Chat Translation Error Detection for Assisting Cross-lingual Communications

In this paper, we describe the development of a communication support system that detects erroneous translations to facilitate crosslingual communications due to the limitations of current machine chat translation methods. We trained an error detector as the baseline of the system and constructed a new Japanese-English bilingual chat corpus, BPersona-chat, which comprises multiturn colloquial chats augmented with crowdsourced quality ratings. The error detector can serve as an encouraging foundation for more advanced erroneous translation detection systems.

==> archived/tab_ablation_accuracy.tex <==
\begin{table}[!t]
\centering
\small
\tabcolsep=3.5pt
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{2}{c}{\textbf{erroneous}} & \multicolumn{2}{c}{\textbf{correct}} \\ %\midrule
\multicolumn{1}{c}{\textbf{classifier}} & \textbf{OS2018} & \textbf{BPchat} & \textbf{OS2018} & \textbf{BPchat} \\ \midrule
1A-1B-2B-2A & 0.9338 & 0.9560 & 0.7246 & 0.9554 \\ \midrule
1A-2B-2A & 0.9292 & 0.9570 & 0.7185 & 0.9499 \\ 
2B-2A & 0.9169 & 0.9453 & 0.7277 & 0.9474 \\%\midrule
1A-2A & 0.9000 & 0.9333 & 0.5862 & 0.9717 \\ %\midrule
\bottomrule
 \end{tabular}
\caption{The accuracy of ablation models on predicting 2A. Note that 1A-1B-2B-2A is identical to the baseline shown in Table~\ref{tab:baseline-accuracy}.
% is model-translated or human-translated with OpenSubtitles2018 (OS2018) and BPersona-chat (BPchat).
}
\label{tab:ablation-accuracy}
%\vspace{-1mm}
\end{table}

==> archived/tab_ablation_score.tex <==
\begin{table}[t]
\centering
\small
\tabcolsep 3pt
\begin{tabular}{@{}lllllll@{}}
\toprule
%& \multicolumn{3}{c}{\textbf{BPchat}} & \multicolumn{3}{c}{\textbf{OS2018}} \\
& \multicolumn{3}{c}{\textbf{ja $\rightarrow$ en}} & \multicolumn{3}{c}{\textbf{en $\rightarrow$ ja}} \\
&
  \multicolumn{1}{c}{\textbf{F}} &
  \multicolumn{1}{c}{(\textbf{Pre}} &
  \multicolumn{1}{c}{\textbf{Rec})} &
  \multicolumn{1}{c}{\textbf{F}} &
  \multicolumn{1}{c}{(\textbf{Pre}} &
  \multicolumn{1}{c}{\textbf{Rec})} \\ \midrule
%1A1B2B-2A & \textbf{95.57} & (95.55 & 95.60) & \textbf{84.54} & (77.22 & 93.38) \\ \midrule
%1A2B-2A & 95.36 & (95.02 & 95.70) & 84.06 & (76.75 & 92.92) \\ % 1A-2B-2A
%2B-2A  & 94.63 & (94.73 & 94.53) & 83.77 & (77.10 & 91.69) \\ % 2B-2A
%1A-2A  & 95.15 & (97.06 & 93.33) & 77.79 & (68.50 & 90.00) \\ % 1A-2A
1A1B2B-2A & \textbf{89.08} & (83.58 & 95.34) & 90.16 & (83.71 & 97.67) \\ \midrule
1A2B-2A & 88.59 & (82.94 & 95.06) & 89.53 & (82.27 & 98.19) \\ % 1A-2B-2A
2B-2A  & 88.58 & (86.69 & 95.37) & 84.75 & (75.84 & 96.04) \\ % 2B-2A
1A-2A  & 88.44 & (86.62 & 90.32) & \textbf{90.48} & (84.60 & 97.24) \\ % 1A-2A
\bottomrule
\end{tabular}
%\caption{The performance of our baseline model (1A1B2B) and ablated models (1A2B, 2B, and 1A) in F-score, precision, and recall on BPersona-chat and OpenSubtitles2018.}
\caption{The performance of our baseline model (1A1B2B-2A) and ablated models (1A2B, 2B, and 1A) in F-score, precision, and recall on BPersona-chat.}
\label{tab:ablation-score}
\end{table}

==> archived/tab_chat_1A2B2A_2.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{1A} & He is a shithead.                   \\ \midrule
\textbf{2B} & 毎年、彼は息子の誕生日を忘れるの    \\ \midrule
\textbf{2A} & (translated) Every year he forgets his birthday. \\
            & (reference) Every year he forgets his son's birthday. \\ \bottomrule
\end{tabular}
\caption{An example of chat with an erroneous 2A.}
\label{tab:chat-1A2B2A-2}
%\vspace{-1mm}
\end{table}

==> archived/tab_confusion_matrix_enja.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\small
\tabcolsep 3pt
\begin{tabular}{@{}lcclcclcc@{}}
\toprule
\multicolumn{3}{c}{\textbf{human}}   & \multicolumn{3}{c}{\textbf{NMT model A}} & \multicolumn{3}{c}{\textbf{NMT model B}}   \\ \midrule
 &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} &
  \textbf{} &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} &
  \textbf{} &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} \\
\textbf{correct} & 2406 & 176 & \textbf{correct} & 6  & 265  & \textbf{correct} & 1005 & 758 \\
\textbf{erroneous} & 83 & 9 & \textbf{erroneous} & 53 & 2350 & \textbf{erroneous} & 505  & 406 \\ \bottomrule
\end{tabular}
\caption{\hl{
The confusion matrix of the error detector on the \textbf{en-to-ja} direction of BPersona-chat. The row headers are the actual annotations, while the column headers are the prediction made by the detector.
}}
\label{tab:confusion-matrix-enja}
\end{table*}

==> archived/tab_confusion_matrix_jaen.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\small
\tabcolsep 3pt
\begin{tabular}{@{}lcclcclcc@{}}
\toprule
\multicolumn{3}{c}{\textbf{human}}   & \multicolumn{3}{c}{\textbf{NMT model A}} & \multicolumn{3}{c}{\textbf{NMT model B}}   \\ \midrule
 &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} &
  \textbf{} &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} &
  \textbf{} &
  \multicolumn{1}{l}{\textbf{correct}} &
  \multicolumn{1}{l}{\textbf{erroneous}} \\
\textbf{correct} & 2677 & 312 & \textbf{correct} & 11  & 155  & \textbf{correct} & 1792 & 827 \\
\textbf{erroneous}   & 290   & 21   & \textbf{erroneous}   & 90 & 2140 & \textbf{erroneous}   & 374  & 181 \\ \bottomrule
\end{tabular}
\caption{\hl{
The confusion matrix of the error detector on the \textbf{ja-to-en} direction of BPersona-chat. The row headers are the actual annotations, while the column headers are the prediction made by the detector.
}}
\label{tab:confusion-matrix-jaen}
\end{table*}
